Motion Planning for Hybrid Dynamical Systems: Framework, Algorithm Template, and a Sampling-based Approach

This paper focuses on the motion planning problem for the systems exhibiting both continuous and discrete behaviors, which we refer to as hybrid dynamical systems. Firstly, the motion planning problem for hybrid systems is formulated using the hybrid equation framework, which is general to capture most hybrid systems. Secondly, a propagation algorithm template is proposed that describes a general framework to solve the motion planning problem for hybrid systems. Thirdly, a rapidly-exploring random trees (RRT) implementation of the proposed algorithm template is designed to solve the motion planning problem for hybrid systems. At each iteration, the proposed algorithm, called HyRRT, randomly picks a state sample and extends the search tree by flow or jump, which is also chosen randomly when both regimes are possible. Through a definition of concatenation of functions defined on hybrid time domains, we show that HyRRT is probabilistically complete, namely, the probability of failing to find a motion plan approaches zero as the number of iterations of the algorithm increases. This property is guaranteed under mild conditions on the data defining the motion plan, which include a relaxation of the usual positive clearance assumption imposed in the literature of classical systems. The motion plan is computed through the solution of two optimization problems, one associated with the flow and the other with the jumps of the system. The proposed algorithm is applied to an actuated bouncing ball system and a walking robot system so as to highlight its generality and computational features.

==> macros/commands.tex <==
\newcommand{\pn}[1]{{\color{red} #1}}
\newcommand{\pnn}[1]{{\color{blue} #1}}
\newcommand{\pno}[1]{{\color{cyan} #1}}

\newcommand{\Reals}[1][]{\mathbb{R}^{#1}}
\newcommand{\Preals}[1][]{\mathbb{R}^{#1}_{\geq 0}}

\newbool{conf}
\setbool{conf}{false}

\ifbool{conf}{
% Items for conference version go in here.
}{
% Items for report version go in here.
 \addtolength{\oddsidemargin}{-.875in}
	\addtolength{\evensidemargin}{-.875in}
	\addtolength{\textwidth}{1.75in}
	\addtolength{\topmargin}{-.875in}
	\addtolength{\textheight}{1.75in} 
}

==> macros/packages.tex <==
\usepackage{./macros/hslTR}

\usepackage{graphics}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{verbatim}     
\usepackage{amsxtra}
\usepackage{epsfig}
\usepackage{subfigure}
\usepackage{hyperref} 
\usepackage{amsmath}
\usepackage{latexsym}
\usepackage{ifthen}
\usepackage{psfrag}
\usepackage{subfigure}
\usepackage{color}
\usepackage{float}
\usepackage{tikz}
\usepackage{mathtools}
\usepackage{etoolbox}
\usepackage{enumitem}

\usepackage{./macros/rgsEnvironments}
\usepackage{./macros/rgsMacros}  

\usepackage{algorithm}
\usepackage{algpseudocode}

\usetikzlibrary{shapes,arrows}

==> macros/theorems.tex <==
 \newcounter{theorem}
\newtheorem{problem}[theorem]{Problem}

\newcommand{\incfig}[2][1]{%
	\def\svgwidth{#1\columnwidth}
	\import{./figures/}{#2.pdf_tex}
}

\DeclareMathOperator{\interior}{int}
\DeclareMathOperator*{\argmin}{arg\,min}

\newlist{steps}{enumerate}{1}
\setlist[steps, 1]{leftmargin=45pt, label = \textbf{Step \arabic*}:}

==> sections/algorithmtemplate/backwardintimesystem.tex <==
\subsection{Backward-in-time Hybrid Systems}
In the proposed template, a backward-in-time version of the hybrid system $\mathcal{H} = (C, f, D, g)$, denoted $\mathcal{H}^{\text{bw}} = (C^{\text{bw}}, f^{\text{bw}}, D^{\text{bw}}, g^{\text{bw}})$, is required when propagating trajectories backward in hybrid time. The backward-in-time hybrid system $\mathcal{H}^{\text{bw}}$ is constructed as follows.
\begin{definition}
	(Backward-in-time hybrid system) Given a hybrid system $\mathcal{H} = (C, f, D, g)$, the backward-in-time hybrid system of $\mathcal{H}$, denoted $\mathcal{H}^{\text{bw}}$, is the hybrid system
	\begin{equation}
	\mathcal{H}: \left\{              
	\begin{aligned}               
	\dot{x} & =  f^{\text{bw}}(x, u)     &(x, u)\in C^{\text{bw}}\\                
	x^{+} & \in  g^{\text{bw}}(x, u)      &(x, u)\in D^{\text{bw}}\\                
	\end{aligned}   \right. 
	\label{model:generalhybridbackwardsystem}
	\end{equation}
	where
	\begin{enumerate}[label = \arabic*)]
		\item The backward-in-time flow set is constructed as
		\begin{equation}
		\label{equation:backwardflowset}
		C^{\text{bw}} := C.
		\end{equation}
		\item The backward-in-time flow map is constructed as
		\begin{equation}
		\label{equation:backwardflow}
		\begin{aligned}
		f^{\text{bw}}(x, u) :=  -f(x, u) \quad \forall (x, u)\in C^{\text{bw}}.
		\end{aligned}
		\end{equation} 
		\item The backward-in-time jump map is constructed as
		\begin{equation}
		\label{set:gbw}
		\begin{aligned}
		g^{\text{bw}}(x, u) := \{z\in \mathbb{R}^{n}:\  x = g(z, u), (z, u)\in D\}\\
		 \quad \forall (x, u)\in \mathbb{R}^{n}\times \mathbb{R}^{m}.
		\end{aligned}
		\end{equation}
		\item The backward-in-time jump set is constructed as
		\begin{equation}
		\label{set:dbw}
		\begin{aligned}
		D^{\text{bw}} := \{(x, u)\in \mathbb{R}^{n}\times \mathbb{R}^{m}: \\
		\exists z\in g^{\text{bw}} (x, u): 
		(z, u)\in D\}.
		\end{aligned}
		\end{equation}
	\end{enumerate}
\end{definition}
The above shows a general method of constructing the backward-in-time system given the forward-in-time hybrid system. Note that although the jump map $g$ in the forward-in-time system $\mathcal{H}$  is a single-valued map, the jump map $g^{\text{bw}}$ in the backward-in-time system $\mathcal{H^{\text{bw}}}$ is not necessarily single valued. Hence, a difference inclusion is used in (\ref{model:generalhybridbackwardsystem}). 

The backward-in-time hybrid system of the hybrid system in Example \ref{example:bouncingball} is constructed next. 
\begin{example}\label{example:bouncingballbw}
	(Actuated bouncing ball system in Example \ref{example:bouncingball}, revisited) The backward-in-time hybrid system of the actuated bouncing ball system is constructed as follows.
	\begin{itemize}
		\item From (\ref{equation:backwardflowset}), the backward-in-time flow set $C^{\text{bw}}$ is given by
		\begin{equation}
		\label{equation:bouncingballbwflowset}
		C^{\text{bw}} := C =  \{(x, u)\in \mathbb{R}^{2}\times \mathbb{R}: x_{1} \geq 0\}.
		\end{equation}
		\item From (\ref{equation:backwardflow}), the backward-in-time flow map $f^{\text{bw}}$ is given by
		\begin{equation}
		\label{equation:bouncingballbwflowmap}
		f^{\text{bw}}(x, u) := -f(x, u) = \left[ \begin{matrix}
		-x_{2} \\
		\gamma
		\end{matrix}\right] \qquad (x, u)\in C^{\text{bw}}.
		\end{equation}
		\item From (\ref{set:dbw}), the backward-in-time jump set is given by
		\begin{equation}
		\label{equation:bouncingballbwjumpset}
		D^{\text{bw}} := \{(x, u)\in \mathbb{R}^{2}\times \mathbb{R}: x_{1} = 0, x_{2} \geq u, u\geq 0\}. 
		\end{equation}
		\item From (\ref{set:gbw}), the backward-in-time jump map $g^{\text{bw}}$ is given by 
		\begin{equation}
		\label{equation:bouncingballbwjumpmap}
		g^{\text{bw}}(x, u) :=  \left[ \begin{matrix}
		x_{1} \\
		-\frac{x_{2}}{\lambda}+\frac{u}{\lambda}
		\end{matrix}\right] \qquad (x, u)\in D^{\text{bw}}.
		\end{equation}
	\end{itemize}
	%	In conclusion, the backward-in-time hybrid system is given by:
	%	\begin{equation}
	%	\cal{H}^{\text{bw}}: \left\{              
	%	\begin{aligned}               
	%	\dot{x} &= f^{\text{bw}}(x, u)    &(x, u)\in C^{\text{bw}}\\                
	%	x^{+} &=  g^{\text{bw}}(x, u)    &(x, u)\in D^{\text{bw}}\\                
	%	\end{aligned}   \right.   
	%	\label{model:bouncingballbw}
	%	\end{equation}
	%	where the flow map $f$ is given in (\ref{equation:bouncingballbwflowmap}), the flow set $C$ is given in (\ref{equation:bouncingballbwflowset}), the jump map $g$ is given in (\ref{equation:bouncingballbwjumpmap}) and the jump set $D$ is given in (\ref{equation:bouncingballbwjumpset}).
\end{example}


Proposition \ref{theorem:reversedarcbwsystem} shows that the reversal of the solution pair to a hybrid system is a solution pair to its backward-in-time hybrid system.

\begin{proposition}
	\label{theorem:reversedarcbwsystem}
	Given a hybrid system $\mathcal{H}$ and its backward-in-time system $\mathcal{H^{\text{bw}}}$, if $\psi = (\phi, u)$ is a compact solution pair to $\mathcal{H}$, the reversal $\psi' = (\phi', u')$ of $\psi = (\phi, u)$ is a compact solution pair to $\mathcal{H}^{\text{bw}}$.
\end{proposition}

==> sections/algorithmtemplate/constructmotion.tex <==
\subsection{Construction of Motion Plans}
In the proposed template, reversal and concatenation operations are executed to build motion plans. The two operations are formalized in Definition \ref{definition:reversedhybrdarc} and Definition \ref{definition:concatenation}. Proposition \ref{theorem:reversedarcbwsystem} has shown that the reversal of a solution pair to a hybrid system is a solution pair to its backward-in-time system. Proposition \ref{theorem:concatenationsolution}  below shows that the concatenation of solution pairs satisfies the definition of the solution pair in Definition \ref{definition:solution} under mild conditions.
\begin{proposition}
	\label{theorem:concatenationsolution}
	Given two solution pairs $\psi_{1} = (\phi_{1}, u_{1})$ and $\psi_{2} = (\phi_{2}, u_{2})$ to a hybrid system $\mathcal{H}$, their concatenation $\psi = (\phi, u) = (\phi_{1}|\phi_{2}, u_{1}|u_{2})$, denoted $\psi = \psi_{1}|\psi_{2}$,  is a solution pair to $\mathcal{H}$ if the following hold:
	\begin{enumerate}[label = \arabic*)]
		\item $\psi_{1} = (\phi_{1}, u_{1})$ is compact;
		\item $\phi_{1}(T, J) = \phi_{2}(0,0)$, where $(T, J) = \max \dom \psi_{1}$;
		\item If both $I_{\psi_{1}}^{J}$ and $I_{\psi_{2}}^{0}$ have nonempty interior, where $I_{\psi}^{j} = \{t: (t, j)\in \dom \psi\}$ and $(T, J) = \max \dom \psi_{1}$, then $\psi_{2}(0, 0)\in C$.
		%\item \color{red}$(0, 0)\to u_{2}(0, 0)$ is Lebesgue measurable and bounded. \color{black}
	\end{enumerate}
\end{proposition}
\begin{remark}
		Item 1 in Proposition \ref{theorem:concatenationsolution} guarantees that $\psi_{2}$ can be concatenated to $\psi_{1}$. Definition \ref{definition:concatenation} suggests that if $\psi_{2}$ can be concatenated to $\psi_{1}$, $\psi_{1}$ is required to be compact. 
		Item 2 in Proposition \ref{theorem:concatenationsolution} guarantees that the concatenation $\psi$ satisfies items 1a and 2 in Definition \ref{definition:solution} at hybrid time $(T, J)$, where $(T, J) = \max \dom \psi_{1}$.
		Item 3 in Proposition \ref{theorem:concatenationsolution} guarantees that the concatenation result $\psi$ satisfies item 1b in Definition \ref{definition:solution} at hybrid time $(T, J)$, where $(T, J) = \max \dom \psi_{1}$. Note that item 1b therein does not require that $\psi_{1}(T, J)\in C$ and $\psi_{2}(0,0)\in C$ since $T\notin \interior I_{\psi_{1}}^{J}$ and $0\notin \interior I_{\psi_{2}}^{0}$. However, $T$ may belong to the interior of $I_{\psi}^{J}$ after concatenation. Hence, Item 3 guarantees that if $T$ belongs to the interior of $I_{\psi}^{J}$ after concatenation, then item 1b in Definition \ref{definition:solution} is still satisfied for $\psi$. 
		$\hfill \blacktriangle$
\end{remark}
The following assumption is imposed on the solution pairs that are used to construct motion plans in the forthcoming forward/ backward propagation algorithm template. 
\begin{assumption}
	\label{assumption:theoreticalcondition}
	Given a solution pair $\psi_{1} = (\phi_{1}, u_{1})$ to a hybrid system $\mathcal{H} = (C, f, D, g)$ and a solution pair $\psi_{2} = (\phi_{2}, u_{2})$ to the backward-in-time hybrid system $\mathcal{H^{\text{bw}}}$ associated to $\mathcal{H}$, the following hold:
	\begin{enumerate}[label = \arabic*)]
		\item $\psi_{1} $ and $\psi_{2} $ are compact;
		\item $\phi_{1}(T_{1}, J_{1}) = \phi_{2}(T_{2}, J_{2})$, where $(T_{1}, J_{1}) = \max \dom \psi_{1}$ and $(T_{2}, J_{2}) = \max \dom \psi_{2}$;
		\item If both $I_{\psi_{1}}^{J_{1}}$ and $I_{\psi_{2}}^{J_{2}}$ have nonempty interior, where $I^{j}_{\psi} =\{t: (t, j)\in \dom \psi\}$, $(T_{1}, J_{1}) = \max \dom \psi_{1}$, and $(T_{2}, J_{2}) = \max$ $\dom \psi_{2}$, then $\psi_{2}(T_{2}, J_{2}) \in C$.
	\end{enumerate}
\end{assumption}
\begin{remark}
	Given a hybrid system $\mathcal{H}$, its backward-in-time system $\mathcal{H}^{\text{bw}}$, a solution pair $\psi_{1}$ to $\mathcal{H}$, and a solution pair $\psi_{2}$ to $\mathcal{H^{\text{bw}}}$, Assumption \ref{assumption:theoreticalcondition} is imposed on $\psi_{1}$ and $\psi_{2}$ to guarantee that the concatenation of the reversal of $\psi_{2}$ to $\psi_{1}$ is a solution pair to $\mathcal{H}$. 
Assumption \ref{assumption:theoreticalcondition} guarantees that the conditions needed to apply Proposition \ref{theorem:reversedarcbwsystem} and Proposition  \ref{theorem:concatenationsolution} hold. Note that conditions that guarantee the existence of nontrivial solutions have been proposed in Proposition 3.4 in \cite{chai2018forward}. For the propagation with parameters $(X_{0}, X_{u}, (C, f, D, g))$, if $\xi \in X_{0}$ is such that\footnote{Given a jump set $D\subset \mathbb{R}^{n}\times \mathbb{R}^{m}$, define $\Pi(D):= \{x\in \mathbb{R}^{n}: \exists u\in U_{D}, \text{s.t. } (x, u)\in D\}$ as the projection of $D$ onto $\mathbb{R}^{n}$, where $U_{D} := \{u\in \mathbb{R}^{m}: \exists x\in \mathbb{R}^{n}\text{ such that } (x, u)\in D\}$} $\xi \in \Pi(D)$ or there exist $\epsilon > 0$, an absolutely continuous function $z:[0, \epsilon] \to \mathbb{R}^{n}$ with $z(0) = \xi$, and a Lebesgue measurable and locally essentially bounded function\footnote{Given a flow set $C\subset \mathbb{R}^{n}\times \mathbb{R}^{m}$, the set denoted $U_{C}$, includes all possible input values that can be applied during flows and is defined as $U_{C} := \{u\in \mathbb{R}^{n}: \exists x\in \mathbb{R}^{n}\text{ such that } (x, u)\in C\}$.} $\tilde{u} : [0, \epsilon] \to U_{C}$ such that $(z(t),\tilde{u}(t))\in C$ for all $t\in (0,\epsilon)$ and $\frac{\text{d}}{\text{d} t}z(t) = f(z(t), \tilde{u}(t))$ for almost all $t \in [0, \epsilon]$, where\footnote{Given a flow set $C\subset \mathbb{R}^{n}\times \mathbb{R}^{m}$, the set-valued maps $\Psi^{u}_{c}: \mathbb{R}^{n} \to U_{C}$ is defined for each $x\in \mathbb{R}^{n}$ as $\Psi^{u}_{c}(x):=\{ u \in U_{C}: (x, u)\in C\}$.} $\tilde{u}(t)\in \Psi^{u}_{c}(z(t))$ for every $t\in [0, \epsilon]$,
then the existence of nontrivial solution pairs is guaranteed from $\xi$. 
Items 2 and 3 in Assumption \ref{assumption:theoreticalcondition} relate the final states and their "last" interval of flow of the given solution pairs.\EndRemark
\end{remark}

 The following result validates that a solution pair constructed using solution pairs satisfying Assumption \ref{assumption:theoreticalcondition} satisfies Definition \ref{definition:solution}. 
\begin{lemma}
		\label{lemma:reverseconcatenation}
		Given a hybrid system $\mathcal{H}$ and its backward-in-time hybrid system $\mathcal{H^{\text{bw}}}$, if $\psi_{1}$ is a solution pair to $\mathcal{H}$ and $\psi_{2}$ is a solution pair to $\mathcal{H^{\text{bw}}}$ such that $\psi_{1}$ and $\psi_{2}$ satisfy Assumption \ref{assumption:theoreticalcondition},  then the concatenation $\psi = \psi_{1}|\psi_{2}'$ is a solution pair to $\mathcal{H}$, where $\psi'_{2}$ is the reversal of $\psi_{2}$.
	\end{lemma}
		\begin{proof}
			\input{sections/algorithmtemplate/proof_constructionlemma.tex}
		\end{proof}

Lemma \ref{lemma:reverseconcatenation} is exploited by our forthcoming algorithm template, which also checks numerically if Assumption \ref{assumption:theoreticalcondition} holds.

==> sections/algorithmtemplate/proof_constructionlemma.tex <==
According to Definition \ref{definition:reversedhybrdarc}, the reversal operation is executable on $\psi_{2}$ when $\psi_{2}$ is compact. The first condition in Assumption \ref{assumption:theoreticalcondition} guarantees that $\psi_{2}$ is compact. According to Proposition \ref{theorem:reversedarcbwsystem}, the reversal $\psi'_{2}$ of $\psi_{2}$ is a solution pair to $\mathcal{H}$.
	
	Next, we show that the conditions in Proposition \ref{theorem:concatenationsolution} are satisfied.
	\label{remark:assumption}
	\begin{enumerate}[label = \arabic*)]
		\item The first condition in Assumption \ref{assumption:theoreticalcondition} shows that $\psi_{1}$ is compact. Therefore, the first condition in Proposition \ref{theorem:concatenationsolution} is satisfied.
		\item Note that the second condition in Assumption \ref{assumption:theoreticalcondition} suggests that $\phi_{1}(T_{1}, J_{1}) = \phi_{2}(T_{2}, J_{2})$. Since $\phi'_{2}(0, 0) =  \phi_{2}(T_{2}, J_{2})$,  then $\phi_{1}(T_{1}, J_{1}) = \phi'_{2}(0, 0)$ is satisfied. Hence, $\psi_{1}$ and $\psi'_{2}$ satisfy the second condition in Proposition \ref{theorem:concatenationsolution}.
		\item Since $I_{\psi_{2}}^{J_{2}} = I_{\psi'_{2}}^{0}$ and $\psi_{2}(T_{2}, J_{2}) = \psi'_{2}(0, 0)$, then the third condition in Assumption \ref{assumption:theoreticalcondition} implies that $\psi_{1}$ and $\psi'_{2}$ satisfy the third condition in Proposition \ref{theorem:concatenationsolution}.
	\end{enumerate}
	Since the conditions in Proposition \ref{theorem:concatenationsolution} are satisfied, Proposition \ref{theorem:concatenationsolution} guarantees that the concatenation of $\psi'_{2}$ to $\psi_{1}$ is a solution pair to $\mathcal{H}$.

==> sections/operations/main.tex <==
 \subsection{Concatenation operation}
The operations related to our algorithm template include reversal and concatenation operations of solution pairs. 
\begin{definition}
		\label{definition:reversedhybrdarc}
	(Reversal of a solution pair) Given a compact solution pair $(\phi, u)$ to $\mathcal{H} = (C, f, D, g)$, where $\phi: \dom \phi \to \mathbb{R}^{n}$, $u: \dom u \to \mathbb{R}^{m}$, and $(T, J) = \max \dom (\phi, u)$, the pair $(\phi', u')$ is the reversal of $(\phi, u)$, where $\phi': \dom \phi' \to \mathbb{R}^{n}$ with $\dom \phi' \subset \mathbb{R}_{\geq 0}\times \mathbb{N}$ and $u': \dom u' \to \mathbb{R}^{m}$ with $\dom u' = \dom \phi'$,  if the following hold:
	\begin{enumerate}[label = \arabic*)]
		\item  The function $\phi'$ is defined as
		\begin{enumerate}[label = \alph*)]
			\item $\dom \phi' = \{(T, J)\} - \dom \phi$, where the minus sign denotes Minkowski difference; 
			\item $\phi'(t, j) = \phi(T-t, J - j)$ for all $(t, j)\in \dom \phi'$.
		\end{enumerate}
	\item The function $u'$ is defined as
	\begin{enumerate}[label = \alph*)]
		\item $\dom u' = \{(T, J)\} - \dom u$, where the minus sign denotes Minkowski difference; 
		\item For all $j\in \mathbb{N}$ such that $I^{j} = \{t: (t, j)\in \dom u'\}$ has nonempty interior, 
		\begin{enumerate}[label = \roman*)]
			\item For all $t\in \interior I^{j}$,
			$
			u'(t, j) = u(T-t, J - j);
			$
			\item If $I^{0}$ has nonempty interior, then $u'(0, 0)\in \mathbb{R}^{m}$ is such that 
			$
			(\phi'(0, 0), u'(0, 0))\in \overline{C};
			$
			\item For all $t\in \partial I^{j}$ such that $(t, j + 1)\notin \dom u'$ and $(t, j) \neq (0, 0)$,
			$
			u'(t, j)\in \mathbb{R}^{m}.
			$
		\end{enumerate}
		\item For all $(t, j)\in \dom u'$ such that $(t, j + 1)\in \dom u'$,
$
	u'(t, j) = u(T- t, J - j -1).
	$
%	\begin{equation}
%	u'(t, j) \left\{\begin{aligned}
%	&\textcolor{red}{=}u(T-t, J - j) &\text{if }t\in \interior I^{j}\\
%	&\textcolor{red}{\in \mathbb{R}^{m}} &\text{if }t\notin \interior I^{j} \text{and } \\&&(t, j + 1)\notin \dom u'.
%	\end{aligned}\right. 
%	\end{equation}
	\end{enumerate}
	\end{enumerate}
\end{definition}
The reversal of a given solution pair is not always unique, since $u'(t, j)\in \mathbb{R}^{m}$ in item 2b\romannumeral3\ in Definition \ref{definition:reversedhybrdarc} is free. The value assigned to $u'$ at such hybrid time can be given by the continuous extension of $u'$ at $(t, j)$ in the interval $I^{j}$, if it exists.
\begin{definition}
	\label{definition:concatenation}
	(Concatenation operation) Given two functions $\phi_{1}: \dom \phi_{1} \to \mathbb{R}^{n}$ and $\phi_{2}:\dom \phi_{2} \to \mathbb{R}^{n}$, where $\dom \phi_{1}$ and $\dom \phi_{2}$ are hybrid time domains, $\phi_{2}$ can be concatenated to $\phi_{1}$ if $ \phi_{1}$ is compact and $\phi: \dom \phi \to \mathbb{R}^n$ is the concatenation of $\phi_{2}$ to $\phi_{1}$, denoted $\phi = \phi_{1}|\phi_{2}$, namely,
	\begin{enumerate}[label = \arabic*)]
		\item $\dom \phi = \dom \phi_{1} \cup (\dom \phi_{2} + \{(T, J)\}) $, where $(T, J) = \max$ $\dom \phi_{1}$ and the plus sign denotes Minkowski addition;
		\item $\phi(t, j) = \phi_{1}(t, j)$ for all $(t, j)\in \dom \phi_{1}\backslash \{(T, J)\}$ and $\phi(t, j) = \phi_{2}(t - T, j - J)$ for all $(t, j)\in \dom \phi_{2} + \{(T, J)\}$.
	\end{enumerate}
\end{definition}
The truncation operation of the solution pair is used in the proofs of the main results. The definition of the truncation operation is given as follows.
\begin{definition}
	\label{definition: truncation}
	(Truncation and translation operation) Given a function $\phi: \dom \phi \to \mathbb{R}^{n}$, where $\dom \phi$ is a hybrid time domain, and pairs of hybrid time $(T_{1}, J_{1})\in \dom \phi$ and $(T_{2}, J_{2})\in \dom \phi$ such that $T_{1}\leq T_{2}$ and $J_{1} \leq J_{2}$, the function $\widetilde\phi: \dom \widetilde\phi \to \mathbb{R}^{n}$ is the truncation of $\phi$ between $(T_{1}, J_{1})$ and $(T_{2}, J_{2})$ and translation by $(T_{1}, J_{1})$  if
	\begin{enumerate}[label = \arabic*)]
		%	\item $\max_{t}\dom \widetilde\phi = T$, $\max_{j}\dom \widetilde\phi = J$;
		\item $\dom \widetilde\phi =  (\dom \phi \cap ([T_{1}, T_{2}]\times \{J_{1}, J_{1} + 1, ..., J_{2}\})) - \{(T_{1}, J_{1})\}$, where the minus sign denotes Minkowski difference;
		\item $\widetilde\phi(t, j) = \phi(t + T_{1}, j + J_{1})$ for all $(t, j)\in \dom \widetilde\phi$.
	\end{enumerate}
\end{definition}

==> sections/preliminaries/truncation.tex <==
\begin{definition}
	\label{definition: truncation}
	(Truncation and translation operation) Given a function $\phi: \dom \phi \to \mathbb{R}^{n}$, where $\dom \phi$ is hybrid time domain, and pairs of hybrid time $(T_{1}, J_{1})\in \dom \phi$ and $(T_{2}, J_{2})\in \dom \phi$ such that $T_{1}\leq T_{2}$ and $J_{1} \leq J_{2}$, the function $\widetilde\phi: \dom \widetilde\phi \to \mathbb{R}^{n}$ is the truncation of $\phi$ between $(T_{1}, J_{1})$ and $(T_{2}, J_{2})$ and translation by $(T_{1}, J_{1})$  if
	\begin{enumerate}
		%	\item $\max_{t}\dom \widetilde\phi = T$, $\max_{j}\dom \widetilde\phi = J$;
		\item $\dom \widetilde\phi =  \dom \phi \cap ([T_{1}, T_{2}]\times \{J_{1}, J_{1} + 1, ..., J_{2}\}) - \{(T_{1}, J_{1})\}$, where the minus sign denotes Minkowski difference;
		\item $\widetilde\phi(t, j) = \phi(t + T_{1}, j + J_{1})$ for all $(t, j)\in \dom \widetilde\phi$.
	\end{enumerate}
\end{definition}

==> sections/validation/main.tex <==
In the proposed algorithm, the concatenation operations are executed heavily to build motion plans. The concatenation operation on hybrid arcs is formalized in Definition \ref{definition:concatenation}. Proposition \ref{theorem:concatenationsolution} below shows that the concatenation of solution pairs satisfies the definition of the solution pair in Definition \ref{definition:solution} under mild conditions.
\begin{proposition}
	\label{theorem:concatenationsolution}
	Given two solution pairs $\psi_{1} = (\phi_{1}, u_{1})$ and $\psi_{2} = (\phi_{2}, u_{2})$ to a hybrid system $\mathcal{H}$, their concatenation $\psi = (\phi, u) = (\phi_{1}|\phi_{2}, u_{1}|u_{2})$, denoted $\psi = \psi_{1}|\psi_{2}$,  is a solution pair to $\mathcal{H}$ if the following hold:
	\begin{enumerate}[label = \arabic*)]
		\item $\psi_{1} = (\phi_{1}, u_{1})$ is compact;
		\item $\phi_{1}(T, J) = \phi_{2}(0,0)$, where $(T, J) = \max \dom \psi_{1}$;
		\item If both $I_{\psi_{1}}^{J}$ and $I_{\psi_{2}}^{0}$ have nonempty interior, where $I_{\psi}^{j} = \{t: (t, j)\in \dom \psi\}$ and $(T, J) = \max \dom \psi_{1}$, then $\psi_{2}(0, 0)\in C$.
		%\item \color{red}$(0, 0)\to u_{2}(0, 0)$ is Lebesgue measurable and bounded. \color{black}
	\end{enumerate}
\end{proposition}
